Fast and Robust Video-Based Exercise Classification via Body Pose Tracking and Scalable Multivariate Time Series Classifiers

Technological advancements have spurred the usage of machine learning based applications in sports science. Physiotherapists, sports coaches and athletes actively look to incorporate the latest technologies in order to further improve performance and avoid injuries. While wearable sensors are very popular, their use is hindered by constraints on battery power and sensor calibration, especially for use cases which require multiple sensors to be placed on the body. Hence, there is renewed interest in video-based data capture and analysis for sports science. In this paper, we present the application of classifying S\&C exercises using video. We focus on the popular Military Press exercise, where the execution is captured with a video-camera using a mobile device, such as a mobile phone, and the goal is to classify the execution into different types. Since video recordings need a lot of storage and computation, this use case requires data reduction, while preserving the classification accuracy and enabling fast prediction. To this end, we propose an approach named BodyMTS to turn video into time series by employing body pose tracking, followed by training and prediction using multivariate time series classifiers. We analyze the accuracy and robustness of BodyMTS and show that it is robust to different types of noise caused by either video quality or pose estimation factors. We compare BodyMTS to state-of-the-art deep learning methods which classify human activity directly from videos and show that BodyMTS achieves similar accuracy, but with reduced running time and model engineering effort. Finally, we discuss some of the practical aspects of employing BodyMTS in this application in terms of accuracy and robustness under reduced data quality and size. We show that BodyMTS achieves an average accuracy of 87\%, which is significantly higher than the accuracy of human domain experts.

==> Abstract.tex <==
\begin{abstract}
    %-------------------------------------------------------------------------
	%The abstract should briefly summarize the contents of the paper in	about 250-300 words.
	%-------------------------------------------------------------------------
	%1. What is the problem addressed?
    %2. Why is it important?
    %3. Why is it challenging?
    %4. What are the existing solutions and their limitations? 
    %5. What does this paper propose? 
    %6. What are the results/lessons learned so far? 
	%1. What is the problem addressed?

%Requirements: (Sect: abstract + intro; rel work)
%Task: Strength and Conditioning exercise classification: why important, why challenging, gaps (we do not focus on classifying dance motion or other sports)
%Video data capture
%Light computation for training/test
%High accuracy
%Robustness to noise

% Background
Recent technological advancements have spurred the usage of machine learning based applications in sports science and healthcare. Using wearable sensors and video cameras to analyze and improve the performance of athletes, has become widely popular.
Physiotherapists, sports coaches and athletes actively look to incorporate the latest technologies in order to further improve performance and avoid injuries. While wearable sensors are very popular, their use is hindered by constraints on battery power and sensor calibration, especially for use cases which require multiple sensors to be placed on the body. 
Hence, there is renewed interest in video-based data capture and analysis for sports science. 
% Little info about the previous work
%Our previous work \cite{ashish2020} presented a holistic approach (BodyMTSC) for the interpretable classification of Military Press (MP) which is a standard Sports and Conditioning (S\&C) exercise where the objective was to facilitate physiotherapists, sports coaches and rehabilitation patients by providing feedback after the execution of MP.
% BodyMTSC is a lightweight, two-step approach to classify the different executions of Military Press into predefined labels from the videos. 
%Recent work proposed approaches for interpretable video-based classification of a strength and conditioning exercise, the Military Press (MP), where the objective was to facilitate physiotherapists, sports coaches and rehabilitation patients by providing feedback after the exercise execution. The methodology proposed transformed the video into time series data by employing body pose tracking, followed by time series classification methods.
% BodyMTSC is a lightweight, two-step approach to classify the different executions of Military Press into predefined labels from the videos. 
%
% Current work, importance and applications
%The work presented in this paper builds upon the previous work.
In this paper, we present the application of classifying strength and conditioning exercises using video. We focus on the popular Military Press exercise, where the execution is captured with a video-camera using a mobile device, such as a mobile phone, and the goal is to classify the execution into different types. 
%Since the mobile device has limited resources, 
Since video recordings need a lot of storage and computation, this use case requires data reduction, while preserving the classification accuracy and enabling fast  prediction.
To this end, we propose an approach named BodyMTS to turn video into time series by employing body pose tracking, followed by training and prediction using multivariate time series classifiers. We analyze the accuracy and robustness of BodyMTS and show that it is robust to different types of noise caused by either video quality or pose estimation factors. We compare BodyMTS to state-of-the-art deep learning methods which classify human activity directly from videos and show that BodyMTS achieves similar accuracy, but with reduced running time and model engineering effort.
%Additionally, we present the latest results from recent version of OpenPose and new classifiers.
Finally, we discuss some of the practical aspects of employing BodyMTS in this application in terms of accuracy and robustness under reduced data quality and size. We show that BodyMTS achieves an average accuracy of 87\%, which is significantly higher than the accuracy of human domain experts.

% We further present a comparison of BodyMTS to state-of-the-art deep learning methods that classify human activity directly from videos. We show that BodyMTS achieves similar or higher accuracy, with much less computational resources and runtime.
\keywords{video-based exercise classification \and strength and conditioning \and body pose tracking \and
time series classification}
\end{abstract}



% Redo the abstract to reflect the answers to DAMI application paper requirements

==> DAMI_2022-MTS-PoseEstimation-Revised 2 (Copy)/Abstract.tex <==
\begin{abstract}
    %-------------------------------------------------------------------------
	%The abstract should briefly summarize the contents of the paper in	about 250-300 words.
	%-------------------------------------------------------------------------
	%1. What is the problem addressed?
    %2. Why is it important?
    %3. Why is it challenging?
    %4. What are the existing solutions and their limitations? 
    %5. What does this paper propose? 
    %6. What are the results/lessons learned so far? 
	%1. What is the problem addressed?

%Requirements: (Sect: abstract + intro; rel work)
%Task: Strength and Conditioning exercise classification: why important, why challenging, gaps (we do not focus on classifying dance motion or other sports)
%Video data capture
%Light computation for training/test
%High accuracy
%Robustness to noise

% Background
Recent technological advancements have spurred the usage of machine learning based applications in sports science and healthcare. Using wearable sensors and video cameras to analyze and improve the performance of athletes, has become widely popular.
Physiotherapists, sports coaches and athletes actively look to incorporate the latest technologies in order to further improve performance and avoid injuries. While wearable sensors are very popular, their use is hindered by constraints on battery power and sensor calibration, especially for use cases which require multiple sensors to be placed on the body. 
Hence, there is renewed interest in video-based data capture and analysis for sports science. 
% Little info about the previous work
%Our previous work \cite{ashish2020} presented a holistic approach (BodyMTSC) for the interpretable classification of Military Press (MP) which is a standard Sports and Conditioning (S\&C) exercise where the objective was to facilitate physiotherapists, sports coaches and rehabilitation patients by providing feedback after the execution of MP.
% BodyMTSC is a lightweight, two-step approach to classify the different executions of Military Press into predefined labels from the videos. 
%Recent work proposed approaches for interpretable video-based classification of a strength and conditioning exercise, the Military Press (MP), where the objective was to facilitate physiotherapists, sports coaches and rehabilitation patients by providing feedback after the exercise execution. The methodology proposed transformed the video into time series data by employing body pose tracking, followed by time series classification methods.
% BodyMTSC is a lightweight, two-step approach to classify the different executions of Military Press into predefined labels from the videos. 
%
% Current work, importance and applications
%The work presented in this paper builds upon the previous work.
In this paper, we present the application of classifying strength and conditioning exercises using video. We focus on the popular Military Press exercise, where the execution is captured with a video-camera using a mobile device, such as a mobile phone, and the goal is to classify the execution into different types. 
%Since the mobile device has limited resources, 
Since video recordings need a lot of storage and computation, this use case requires data reduction, while preserving the classification accuracy and enabling fast  prediction.
To this end, we propose an approach named BodyMTS to turn video into time series by employing body pose tracking, followed by training and prediction using multivariate time series classifiers. We analyze the accuracy and robustness of BodyMTS and show that it is robust to different types of noise caused by either video quality or pose estimation factors. We compare BodyMTS to state-of-the-art deep learning methods which classify human activity directly from videos and show that BodyMTS achieves similar accuracy, but with reduced running time and model engineering effort.
%Additionally, we present the latest results from recent version of OpenPose and new classifiers.
Finally, we discuss some of the practical aspects of employing BodyMTS in this application in terms of accuracy and robustness under reduced data quality and size. We show that BodyMTS achieves an average accuracy of 87\%, which is significantly higher than the accuracy of human domain experts.

% We further present a comparison of BodyMTS to state-of-the-art deep learning methods that classify human activity directly from videos. We show that BodyMTS achieves similar or higher accuracy, with much less computational resources and runtime.
\keywords{video-based exercise classification \and strength and conditioning \and body pose tracking \and
time series classification}
\end{abstract}



% Redo the abstract to reflect the answers to DAMI application paper requirements
